Fast modeling of turbulent transport in fusion plasmas using neural networks

We present an ultrafast neural network (NN) model, QLKNN, which predicts core tokamak transport heat and particle fluxes. QLKNN is a surrogate model based on a database of 300 million flux calculations of the quasilinear gyrokinetic transport model QuaLiKiz. The database covers a wide range of realistic tokamak core parameters. Physical features such as the existence of a critical gradient for the onset of turbulent transport were integrated into the neural network training methodology. We have coupled QLKNN to the tokamak modelling framework JINTRAC and rapid control-oriented tokamak transport solver RAPTOR. The coupled frameworks are demonstrated and validated through application to three JET shots covering a representative spread of H-mode operating space, predicting turbulent transport of energy and particles in the plasma core. JINTRAC-QLKNN and RAPTOR-QLKNN are able to accurately reproduce JINTRAC-QuaLiKiz T i,e and n e profiles, but 3 to 5 orders of magnitude faster. Simulations which take hours are reduced down to only a few tens of seconds. The discrepancy in the final source-driven predicted profiles between QLKNN and QuaLiKiz is on the order 1%-15%. Also the dynamic behaviour was well captured by QLKNN, with differences of only 4%-10% compared to JINTRAC-QuaLiKiz observed at mid-radius, for a study of density buildup following the L-H transition. Deployment of neural network surrogate models in multi-physics integrated tokamak modelling is a promising route towards enabling accurate and fast tokamak scenario optimization, Uncertainty Quantification, and control applications.

==> Makefile <==
.PHONY: all clean

targets=$(shell for file in `find . -maxdepth 1 -name '*.tex' -type f -printf "%f\n"| sed 's/\..*/\.pdf/'`; do echo "$$file "; done;)

all: $(targets)

figures := $(wildcard Pictures/*)
%.pdf: %.tex main.bbl $(figures)
	latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make $<
	bibtex $(<:.tex=)
	latexmk -g -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make $<

clean:
	        latexmk -CA
	        rm main.bbl

debug:
	@echo $(targets)
	@echo figures: $(shell grep -P 'includegraphics\[.*\]{\K(.*)(?=})' -ro *.tex)

